Vision-Enhanced Time Series Forecasting via Latent Diffusion Models

Diffusion models have recently emerged as powerful frameworks for generating high-quality images. While recent studies have explored their application to time series forecasting, these approaches face significant challenges in cross-modal modeling and transforming visual information effectively to capture temporal patterns. In this paper, we propose LDM4TS, a novel framework that leverages the powerful image reconstruction capabilities of latent diffusion models for vision-enhanced time series forecasting. Instead of introducing external visual data, we are the first to use complementary transformation techniques to convert time series into multi-view visual representations, allowing the model to exploit the rich feature extraction capabilities of the pre-trained vision encoder. Subsequently, these representations are reconstructed using a latent diffusion model with a cross-modal conditioning mechanism as well as a fusion module. Experimental results demonstrate that LDM4TS outperforms various specialized forecasting models for time series forecasting tasks.

==> table/short_term_forecasting.tex <==
% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table*}[!htbp]
% \setlength{\tabcolsep}{2pt}
% \captionsetup{font=small}
%   \centering
%   \caption{Short-term time series forecasting results on M4. The forecasting horizons are in [6, 48] and the three rows provided are weighted averaged from all datasets under different sampling intervals. A lower value indicates better performance. Our full results are in Appendix~\ref{appx:short_term_details} }
%     \begin{tabular}{|cc|cccccccccc|}
%     \toprule
%     \multicolumn{2}{|c|}{Methods} & \multicolumn{1}{c|}{LDM4TS (Ours)} & \multicolumn{1}{c|}{Autoformer} & \multicolumn{1}{c|}{FEDformer} & \multicolumn{1}{c|}{DLinear} & \multicolumn{1}{c|}{Informer} & \multicolumn{1}{c|}{TimesNet} & \multicolumn{1}{c|}{LightTS} & \multicolumn{1}{c|}{CSDI} & \multicolumn{1}{c|}{ScoreGrad} & DiffusionTS \\
%     \midrule
%     \multirow{3}[2]{*}{\begin{sideways}Average\end{sideways}} & SMAPE & 18.669 & 12.909 & 13.16 & \multicolumn{1}{c|}{13.639} & 14.086 & 12.88 & 13.525 & 23.918 & 22.331 & - \\
%           & MASE  & 2.676  & 1.771 & 1.775 & 2.095 & 2.718 & 1.836 & 2.111 & 3.131  & 3.596 \\
%           & OWA & 1.388  & 0.939 & 0.949 & 1.051 & 1.23  & 0.955 & 1.051 & 1.7  & 1.764 & - \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:long_term_results}%
% \end{table*}%
% x
